A realizability-preserving discontinuous Galerkin scheme for entropy-based moment closures for linear kinetic equations in one space dimension

We implement a high-order numerical scheme for the entropy-based moment closure, the so-called M$_N$ model, for linear kinetic equations in slab geometry. A discontinuous Galerkin (DG) scheme in space along with a strong-stability preserving Runge-Kutta time integrator is a natural choice to achieve a third-order scheme, but so far, the challenge for such a scheme in this context is the implementation of a linear scaling limiter when the numerical solution leaves the set of realizable moments (that is, those moments associated with a positive underlying distribution). The difficulty for such a limiter lies in the computation of the intersection of a ray with the set of realizable moments. We avoid this computation by using quadrature to generate a convex polytope which approximates this set. The half-space representation of this polytope is used to compute an approximation of the required intersection straightforwardly, and with this limiter in hand, the rest of the DG scheme is constructed using standard techniques. We consider the resulting numerical scheme on a new manufactured solution and standard benchmark problems for both traditional M$_N$ models and the so-called mixed-moment models. The manufactured solution allows us to observe the expected convergence rates and explore the effects of the regularization in the optimization.

==> sections/.svn/tmp/svn-jUGyPY <==
%!TEX root = ../MMEOptimization.tex

\section{A linear kinetic equation and moment closures}
\label{sec:momapprox}

We begin with the linear kinetic equation we will use to test our algorithm
and a brief introduction to entropy-based moment closures.
More background can be found for example in \cite{Lewis-Miller-1984,
Lev96,Hauck2010} and references therein.

\subsection{A linear kinetic equation}

We consider the following one-dimensional linear kinetic equation for the 
kinetic density $\psi = \psi(t, x, \mu) \ge 0$ in slab geometry,
for time $t > 0$, spatial coordinate
$x \in X = (\xL, \xR) \subseteq \R$, and angle variable
$\mu \in [-1, 1]$:
\begin{align}
\label{eq:FokkerPlanck1D}
\partial_t\psi + \mu \partial_x  \psi + \sig{a} \psi = 
\sig{s}\collision{\psi} + \source,
\end{align}
where $\sig{a}$ are $\sig{s}$ are the absorption and scattering interaction 
coefficients, respectively, which throughout the paper we assume for notational
simplicity to be constants, and $\source$ a source.
The operator $\collisionop$ is a collision operator, which in this paper we
assume to be linear and have the form
\begin{equation}
 \collision{\psi} = \int_{-1}^1 T(\mu, \mu^\prime)
  \psi(t, x, \mu^\prime)~d\mu^\prime 
  - \int_{-1}^1 T(\mu^\prime, \mu) \psi(t, x, \mu)~d\mu^\prime.
\label{eq:collisionOperator}
\end{equation}
We assume that the kernel $T$ is strictly positive and normalized such that 
$\int_{-1}^1 T(\mu^\prime, \mu) d\mu^\prime~\equiv~1$.  A typical example is 
isotropic scattering, where $T(\mu, \mu^\prime) \equiv 1/2$.

Equation \eqref{eq:FokkerPlanck1D} is supplemented by initial and boundary 
conditions:
\begin{subequations}
\label{eq:bc-ic}
\begin{align}
 \psi(t, \xL,\mu) &= \psiL(t, \mu) \:, \quad \mu>0\:, \: t \geq 0 \:, \\
 \psi(t, \xR,\mu) &= \psiR(t, \mu) \:, \quad \mu<0\:, \: t \geq 0 \:,\\
 \psi(0, x,\mu) &= \psiInit(x,\mu)  \:, \quad \mu \in [-1,1] \:, \: x \in 
  (\xL,\xR) \:,
\end{align}
\end{subequations}
where $\psiL$, $\psiR$, and $\psiInit$ are given.

\subsection{Moment equations and entropy-based closures}

Moments are defined by angular averages against a set of basis functions.  
We use the following notation for angular integrals:
$$
 \Vint{g} = \int_{-1}^1 g(\mu) d\mu
$$
for any integrable function $g = g(\mu)$;
and therefore if we collect the basis functions into a vector $\basis = 
\basis(\mu) = (\basisComp_0(\mu), \basisComp_1(\mu), \ldots, 
\basisComp_{\nmom}(\mu))^T$, then the moments of a kinetic density
$\phi = \phi(\mu)$ are given by $\U = \Vint{\basis \phi}$.

Moment equations are partial differential equations of the form
\begin{equation}
 \partial_t \U + \partial_x \bff(\U) + \sig{a}\U = \sig{s} \br(\U) + 
  \Vint{\basis \source},
\label{eq:moment-closure}
\end{equation}
where the moment vector $\U(t, x)$ approximates $\vint{\basis \psi}$ for the 
kinetic density $\psi$ satisfying \eqref{eq:FokkerPlanck1D}.
In an entropy-based closure (commonly referred in standard polynomial 
bases as the $\MN$ model or the Levermore closure after he exposed their
general structure in \cite{Lev96}), the functions $\bff$ and $\br$
have the form
$$
 \bff(\U) := \Vint{\mu \basis \ansatz_{\U}} \quand
 \br(\U)  := \Vint{\basis \collision{\ansatz_{\U}}}.
$$
Here $\ansatz_{\U}$ is an \textit{ansatz} density reconstructed from the
moments  $\U$ by solving the constrained optimization problem:
\begin{equation}
 \ansatz_{\U} = \argmin\limits_\phi \left\{\Vint{\eta(\phi)}
 : \Vint{\basis \phi} = \U \right\},
\label{eq:primal}
\end{equation}
where the kinetic entropy density $\eta$ is strictly convex and
the minimum is simply taken over functions $\phi = \phi(\mu)$ such that 
$\Vint{\eta(\phi)}$ is well defined.
This problem, which must be solved over the space-time mesh, is typically 
solved through its strictly convex finite-dimensional dual,
\begin{equation}
 \alphahat(\U) := \argmin_{\bsalpha \in \R^{\nmom + 1}} \Vint{\eta_*(\basis^T 
  \bsalpha)} - \U^T \bsalpha,
\label{eq:dual}
\end{equation}
where $\eta_*$ is the Legendredual of $\eta$.
The first-order necessary conditions for the $\alphahat(\U)$ 
show that the solution to \eqref{eq:primal} has the form
\begin{equation}
 \ansatz_{\U} = \etad' \left(\basis^T \alphahat(\U) \right)
\label{eq:psiME}
\end{equation}
where $\etad'$ is the derivative of $\eta_*$.


The kinetic entropy density $\eta$ can be chosen according to the 
physics being modelled.
As in \cite{Hauck2010} we use Maxwell-Boltzmann entropy%
\footnote{%
Indeed in a linear setting such as ours, any convex entropy $\eta$ is 
dissipated by \eqref{eq:FokkerPlanck1D}, so we have some freedom.
We focus on the Maxwell-Boltzmann entropy because it is physically relevant for 
many problems, gives a positive ansatz $\ansatz_{\U}$, and also allows
us to explore 
some of the challenges of numerically simulating entropy-based moment closures.%
} %
\begin{align}
\label{eq:EntropyM}
 \eta(z) = z \log(z) - z;
\end{align}
thus $\etad(y) = \etad'(y) = \exp(y)$.


In this paper we consider both the monomial moments, defined by the basis
$$
 \mbasis := \left(1, \mu, \ldots, \mu^{\nmom} \right)^T
$$
and the so-called mixed-moments \cite{SchneiderAlldredge14}, which contain
the usual zeroth-order moment but half moments in the higher orders
This is achieved using the basis functions
$$
\mmbasis(\mu) := \left( 1,
%\mu \mathbbm{1}_{[0, 1]},
%\mu \mathbbm{1}_{[-1, 0]}, 
%\ldots , \mu^\nmom \mathbbm{1}_{[0, 1]}, \mu^\nmom \mathbbm{1}_{[-1, 0]} 
\mu_+,
\mu_-, 
\ldots , \mu^\nmom_+, \mu^\nmom_- 
\right)^T,
$$
where $\nu_+ = \max(\mu, 0)$ and $\nu_- = \min(\mu, 0)$.%
%where $\mathbbm{1}_I$ is the indicator function for interval $I$.%
\footnote{
Notice that in the mixed-moment case, there are $2\nmom + 1$ basis functions 
instead of $\nmom + 1$ as in the monomial case.
However, for clarity of exposition, for most of the paper we will assume 
$\basis$ has $\nmom + 1$ components, though everything applies to the 
mixed-moment case as well.%
} %
Mixed-moment models, which we refer to as MM$_{\nmom}$, have been
introduced to address disadvantages like 
the zero net-flux-problem and unphysical shocks in full-moment models
\cite{Frank07,SchneiderAlldredge14}.



We close this section by quickly noting that the classical P$_{\nmom}$ 
approximation \cite{Lewis-Miller-1984} is an 
entropy-based moment closure by choosing the basis $\basis$ as the Legendre 
polynomials and using the entropy
$$
 \eta(z) = \frac12 z^2.
$$
This results in the ansatz
$$
 \ansatz_{\U} = \basis^T \bsalpha,
$$
which clearly is not necessarily positive.  Nonetheless the resulting moment 
system is linear, simple to compute, and for high values of $\nmom$ provides 
good baseline solutions to the original kinetic equation
\eqref{eq:FokkerPlanck1D}.

\subsection{Moment realizability}

Since the underlying kinetic density we are trying to approximate is
nonnegative, a 
moment vector only makes sense physically if it can be associated with a 
nonnegative density, and in this case the moment vector is called 
\textit{realizable}.
Additionally, since the entropy ansatz has the form \eqref{eq:psiME}, in the 
Maxwell-Boltzmann case the optimization problem \eqref{eq:primal} only has a 
solution if the moment vector lies in the ansatz space
$$
 \cA := \left\{ \Vint{\basis \exp \left( \bsalpha^T \basis \right)} 
  : \bsalpha \in \bbR^{N + 1}  \right\}.
$$
In our case, where the domain of angular integration is bounded, the ansatz 
space $\cA$ is exactly equal to the set of realizable moment vectors 
\cite{Jun00}.
Therefore we can focus simply on realizable moments, so in this section we 
quickly review their characterization in the cases of exact and approximate 
integration.

\subsubsection{Classical theory}\hskip 1pt\\
\label{sec:realizability-thy}


\begin{definition}
The \emph{realizable set} \RD{\basis}{} is 
$$
\RD{\basis}{} = \left\{\U~:~\exists \phi(\mu)\ge 0,\, \Vint{\phi} > 0,
 \text{ such that } \U = \Vint{\basis\phi} \right\}.
$$
Any $\phi$ such that $\U = \vint{\basis \phi}$ is called a \emph{representing 
density}.
\end{definition}

The realizable set is a convex cone.

In the monomial basis $\basis = \mbasis$, a moment vector is realizable if 
and only if its corresponding Hankel matrices are positive definite 
\cite{Shohat-Tamarkin-1943}.
When a moment vector sits exactly on $\partial \RD{\mbasis}{}$, there is only 
one representing density, and it is a linear combination of point masses 
\cite{CurFial91}.
In this case, the corresponding Hankel matrices are singular.
This also causes the optimization problem to be arbitrarily poorly conditioned 
as the moment vector approaches $\partial \RD{\mbasis}{}$
\cite{AllHau12}.

Realizability conditions in the mixed-moment basis $\basis = \mmbasis$ are given 
in \cite{SchneiderAlldredge14} again using Hankel matrices for each half 
interval $[-1, 0]$ and $[0, 1]$ as well as another condition to ``glue'' the 
half-interval conditions together.  In this case, only a subset of the moment 
vectors on $\partial \RD{\mmbasis}{}$ have unique representing densities, but 
those that do include point masses.

\subsubsection{The numerically realizable set}
\label{sec:NumQuad}

In general, angular integrals cannot be computed analytically.  We define a 
quadrature for functions $\phi:[-1,1]\to\R$ by nodes $\{\mu_i\}_{i=1}^{\nQ}$ and 
weights 
$\{w_i\}_{i=1}^{\nQ}$ such that
\begin{align*}
\sum\limits_{i=1}^{\nQ} w_i \phi(\mu_i) \approx \Vint{\phi}
\end{align*}
Below we often abuse notation and write $\Vint{\phi}$ when in 
implementation we mean its approximation by quadrature.
Then as defined in \cite{ahot2013} the numerically realizable set is
$$
\RQ{\basis} = \left\{\U~:~\exists f_i > 0 \text{ s.t. } \U = \sum_{i = 
1}^{\nQ}w_i \basis(\mu_i) f_i \right\} %\label{eq:QRealizable}
$$
Indeed, when replacing the integrals in the optimization problem \eqref{eq:primal} 
with quadrature, a minimizer can only exist when $\U \in \RQ{\basis}$.
It is straightforward to show that, as expected, $\RQ{\basis} \subseteq 
\RD{\basis}{}$.
Furthermore, the closure of $\RQone{\basis}$ is a convex polytope:
\begin{proposition}[\!\!\!\cite{ahot2013}]
For any quadrature $\cQ$ with positive weights $w_i$, and for simplicity 
assuming $\basisComp_0(\mu) \equiv 1$,
\begin{align*}
\RQ{\basis}|_{u_0=1} = 
\interior \co \left\{\basis(\mu_i)\right\}_{i=1}^{\nQ}
\end{align*}
where $\interior$ indicates the interior and $\co$ 
indicates the convex hull.
\end{proposition}

==> sections/.svn/tmp/svn-nn6Hbp <==
%!TEX root = ../MMEOptimization.tex

\section{Realizability-preserving discontinuous Galerkin scheme}
\label{sec:dg}

In this section we introduce our high-order numerical method to simulate the 
moment system \eqref{eq:moment-closure}.  We use the Runge-Kutta 
Discontinuous Galerkin (RKDG) approach \cite{CockburnShuPk,Cockburn1989}
and recent techniques for the 
numerical solution of the defining optimization problem \cite{ahot2013}
\eqref{eq:primal}-\eqref{eq:dual}.  Finally in this section we discuss the 
crucial issue of realizability and our linear scaling limiter to handle 
non-realizable moments in the solution.

\subsection{The discontinuous Galerkin formulation}
\label{sec:DGScheme}
We briefly recall the discontinuous Galerkin method for a general system with 
source term:
\begin{align}
\label{eq:AbbrvSystem}
\partial_t \U + \partial_x \bff(\U) &= \bs(\U),
\end{align}
where in our case $\bs(\U) := \sig{s}\br(\U) - \sig{a}\U + \Vint{\basis 
\source}$.
We follow the approach outlined in a series of papers by Cockburn and Shu
\cite{Cockburn1989,CockburnShuIV,CockburnShuPk,CockburnShuP1,CockburnShuV}.
Let $\{t^\timelvl\}_{\timelvl=0}^{\ntime}$ denote time instants in $[0,T]$ with
$t^\timelvl = \timelvl\Delta t$.
We divide the spatial domain $(\xL, \xR)$ into $\ncells$ cells $I_j = (x_{j - 
1/2}, x_{j + 1/2})$, where the cell edges are given by $x_{j \pm 1/2} = x_j \pm 
\dx / 2$ for cell centers $x_j = \xL + (j - 1 / 2)\dx$, and
$\dx = (\xR - \xL) /  \ncells$. 
We seek approximate solutions $\U_h(t^\timelvl, x)$ in the finite
element space
\[
V_h^k = \{v \in L^1(\xL, \xR): v|_{I_{j}} \in P^k(I_j) \text{ for } 
 j \in \{ 1, \ldots , \ncells \} \}.
\]
where $P^{k}(I)$ is the set of polynomials of degree at most $k$ on the
interval $I$.
We follow the Galerkin approach: replace $\U$ in \eqref{eq:AbbrvSystem} by a 
solution of the form $\U_h \in V_h^k$ then multiply the resulting equation
by basis 
functions $v_h$ of $V_h^k$ and integrate over cell $I_j$ to obtain:
\begin{subequations}
\label{eq:dweakform1}
\begin{align}
 \partial_t \int_{I_j} \U_h(t, x)v_h(x)\,dx
 &+ \bff(\U_h(t, x_{j + 1/2}^-)) v_h(x_{j + 1/2}^-)
  - \bff(\U_h(t, x_{j - 1/2}^+)) v_h(x_{j - 1/2}^+) \nonumber \\
 &-\int_{I_j} \bff(\U_h(t, x)) \partial_x v_h(x)\,dx 
 = \int_{I_j} \bs(\U_h(t, x))v_h(x)\,dx \\
 \label{eq:dweakform1a}
 \int_{I_j} \U_h(0, x)v_h(x)\,dx &= \int_{I_j} \Uzero(x) 
v_h(x)\,dx 
\end{align}
\end{subequations}
where $x_{j \pm 1/2}^-$ and $x_{j \pm 1/2}^+$ denote the limits 
from left and right, respectively, and $\Uzero$ is the initial 
condition.
In order to approximately solve the Riemann problem at the cell-interfaces, the fluxes $\bff(\U_h(x_{j 
+ 1/2}^\pm, t))$ at the points of discontinuity are both replaced by a 
numerical flux $\hat \bff(\U_h(t, x_{j + 1/2}^-), \U_h(t, x_{j + 1/2}^+))$, thus 
coupling the elements with their neighbors \cite{toro2009riemann}.
% The choice of a discontinuous basis implies that our approximate solution 
% $\U_h(t, x)$ may be discontinuous at the cell interfaces $x_{j + 1/2}$.
% In this case the flux $\bff(\U_h(t, x_{j + 1/2}))$ is not well defined. 
% We replace the normal trace by a numerical flux function $\hat\bff(\U_h(t,
% x_{j + 1/2}^-), \U_h(t, x_{j + 1/2}^+))$, thus coupling the elements with 
% their neighbors. This numerical flux function has to be consistent
% ($\hat\bff(\bv,\bv)=\bff(\bv)$), Lipschitz, nondecreasing in the first
% argument and nonincreasing in the second one. Using this flux function, the 
% arising Riemann problems at the cell-interface can be solved (approximately)
% \cite{toro2009riemann}.
Several well-known examples for such a numerical flux $\hat \bff$ exist in the
literature.
In this paper we use the global Lax-Friedrichs flux:
\begin{align*}
 \hat \bff(\bv, \bw) = \dfrac{1}{2} \left( \bff(\bv) + \bff(\bw) - C (\bw - 
\bv) \right),
\end{align*}
The numerical viscosity constant $C$ is taken as the global estimate of the 
absolute value of the largest eigenvalue of the Jacobian
$\partial \bff / \partial \U$.
We use $C = 1$, because
for the moment systems used here it is known that the largest eigenvalue is 
bounded by one in absolute value:
\begin{lemma}
\label{lem:eigenvalues}
The eigenvalues of the Jacobian $\partial \bff / \partial \U$ are bounded
in absolute value by one.
\end{lemma}
\begin{proof}
For convenience, we present a slight generalization of Lemma 4 in 
\cite{Olbrant2012}.

We define $\bJ(\bsalpha) := \Vint{\mu \basis \basis^T \etad''(\basis^T 
\bsalpha)}$ and $\bH(\bsalpha):= \Vint{\basis \basis^T \etad''(\basis^T 
\bsalpha)}$.
Using the properties of $\bH(\bsalpha)$  given in \cite{Lev96},
by applying the chain rule we have
\begin{equation}
 \frac{\partial \bff (\U)}{\partial \U} = \bJ(\alphahat(\U))
 \frac{\partial \alphahat(\U)}{\partial \U}
  = \bJ(\alphahat(\U)) \bH(\alphahat(\U))^{-1}.
\label{eq:fluxJacobian}
\end{equation}
If $\bJ(\alphahat(\U)) \bH(\alphahat(\U))^{-1} \bc = \lambda \bc$ for some 
$\bc \ne 0$, then for $\bd = \bH(\alphahat(\U))^{-1} \bc$ we also have 
$\bJ(\alphahat(\U)) \bd = \lambda \bH(\alphahat(\U)) \bd$, and thus
$$
 |\lambda| \le \frac{\bd^T \bJ(\alphahat(\U)) \bd}{\bd^T \bH(\alphahat(\U)) \bd}
  = \frac{\Vint{\mu \left( \basis^T \bd \right)^2 
  \etad''(\alphahat(\U))}}
  {\Vint{\left( \basis^T \bd \right)^2 \etad''(\alphahat(\U))}} \le 1.
$$
The last inequality follows from the facts that $|\mu| \le 1$ and that 
$\etad'' > 0$, the latter of which is a consequence of the strict 
convexity of $\eta$.
\end{proof}



On each interval, the DG approximate solution $\U_h$ can be written as 
\begin{align}
\label{eqn:solution_form}
\U_h|_{I_j}(t, x) := \U_j(t, x) := \sum_{i=0}^{\order}\Uhat_j^{(i)}(t) 
\varphi_i\left( \frac{x - x_j}{\dx} \right)
\end{align}
where $\{\varphi_0, \varphi_1, \ldots ,\varphi_\order \}$ denote a 
basis for $P^k([-1/2, 1/2])$.
It is convenient to choose an orthogonal basis, so we use Legendre 
polynomials scaled for the interval $[-1/2, 1/2]$:
\begin{align*}
\varphi_0(y) = 1, \quad \varphi_1(y) = 2y, \quad \varphi_2(y) = 
 \frac12 (12y^2-1), \: \ldots
\end{align*}
With an orthogonal basis the cell means $\Ubar_j$ are easily available from the 
expansion coefficients $\Uhat_j$:
$$
\Ubar_j(t) := \frac{1}{\dx} \int_{I_j} \U_j(t, x) dx
 = \frac{1}{\dx} \sum_{i=0}^{\order} \Uhat_j^{(i)}(t)
 \int_{I_j} \varphi_i\left( \frac{x - x_j}{\dx} \right) dx
 = \Uhat_j^{(0)}(t)
$$
We collect the coefficients $\Uhat_j^{(i)}(t)$ into the $(\order + 1) \times 
(\nmom + 1)$ matrix
$$
\Uhat_j(t) = \left( \begin{array}{c}
           \left( \Uhat^{(0)}_j(t) \right)^T \\
           \vdots \\
           \left( \Uhat^{(k)}_j(t) \right)^T
          \end{array} \right)
$$


Using the form of the approximate solution in (\ref{eqn:solution_form}), we can 
write \eqref{eq:dweakform1} in matrix form:
\begin{subequations}
\label{eq:dweakform2}
\begin{align}
\bM \partial_t \Uhat_j + 
\bF(\Uhat_{j - 1}, \Uhat_j, \Uhat_{j + 1}) - 
\bV(\Uhat_j) &= \bS(\Uhat_j) \label{eq:weakform_m1} \\
\left(\bM \Uhat_j(0)\right)_{i\ell} &= 
\int_{I_j} u_{\ell, t = 0}(x) \varphi_i\left( \frac{x - x_j}{\dx} 
\right)  dx \label{eq:weakform_m2}
\end{align}
\end{subequations}
with
\begin{subequations}
\label{eq:weakFormDefs}
\begin{align}
 (\bfM)_{i\ell} =& \int_{I_j} \varphi_i \left( \frac{x - x_j}{\dx} \right)
  \varphi_\ell \left( \frac{x - x_j}{\dx} \right)~dx, \\
 (\bF(\Uhat_{j - 1}(t), \Uhat_j(t), \Uhat_{j + 1})(t))_{i\ell} =& 
  \hat f_{\ell}(\U_j(t, x_{j + 1/2}^-), \U_{j + 1}(t, x_{j + 1/2}^+))
  \varphi_i(1 / 2) \label{eq:numFlux} \\
 & - \hat f_{\ell}(\U_{j - 1}(t, x_{j - 1/2}^-),
  \U_j(t, x_{j - 1/2}^+))\varphi_i(-1 / 2),\\
 (\bV(\Uhat_j(t)))_{i\ell} =& \int_{I_j} f_{\ell}(\U_j(t, x)) \partial_x 
  \varphi_i \left( \frac{x - x_j}{\dx} \right)~dx,\\
 (\bS(\Uhat_j(t)))_{i\ell} =& \int_{I_j} s_{\ell}(\U_j(t, x))
 \varphi_i \left( \frac{x - x_j}{\dx} \right)~dx,
\end{align}
\end{subequations}
where $u_{\ell, t = 0}$, $\hat f_{\ell}$, $f_{\ell}$, and $s_{\ell}$ are the
$\ell$-th components 
of $\Uzero$, $\hat \bff$, $\bff$, and $\bs$ respectively.
Notice that $\bM$ is diagonalized by the choice of an orthogonal basis $\{ 
\varphi_i \}$.
We can write \eqref{eq:weakform_m1} as the ordinary differential equation
\begin{align}
\label{eq:ode1}
\partial_t \Uhat_j &= L_h(\Uhat_{j - 1}, \Uhat_j, \Uhat_{j + 1}), \quad 
\textrm{for } 
j \in \{1, \ldots , \ncells\} \text{ and } t \in (0, T),
\end{align}
with initial condition specified in \eqref{eq:weakform_m2}.

Boundary conditions can be incorporated by adding nonphysical ``ghost'' cells 
at $j = 0$ and $j = \ncells + 1$.
In particular, the quantities $\U_0(t, x_{1/2})$ and $\U_{\ncells + 1}(t, 
x_{\ncells + 1/2})$ used in the numerical flux \eqref{eq:numFlux} in the first 
and last cells are not yet defined.
To define these terms, first we smoothly extend the definitions of
$\psiL(t, \mu)$  and $\psiR(t, \mu)$ to all $\mu$,%
\footnote{
Although this is indeed the most commonly used approach, its inconsistency with 
the original boundary conditions \eqref{eq:bc-ic}, which only specify incoming 
directions, is still an open research topic 
\cite{Pomraning-1964,Larsen-Pomraning-1993-1, 
Larsen-Pomraning-1993-2,Struchtrup-2000,Levermore-2009}.%
}
and then the ghost cells are set to be constant (in space), equal to the 
boundary conditions integrated against the basis functions, so that:
$$
\Uhat_0(t) := \frac{1}{\dx} \left( \begin{array}{c}
                      \Vint{\basis \psiL(t, \cdot)}^T \\ 0 \\ 0
                     \end{array} \right)
 \quand
\Uhat_{\ncells + 1}(t) := \frac{1}{\dx} \left( \begin{array}{c}
                      \Vint{\basis \psiR(t, \cdot)}^T \\ 0 \\ 0
                     \end{array} \right)
$$
% $$
% \U_0(t, x)|_{I_0} := \Vint{\basis \psiL(t, \cdot)}
%  \quand
% \U_{\ncells + 1}(t, x)|_{I_{\ncells + 1}} := \Vint{\basis \psiR(t, \cdot)}.
% $$
This completes the spatial discretization.

In this paper, except for some of the convergence tests in 
\secref{sec:manu-soln}, we use quadratic polynomials ($k = 2$) resulting in a 
third-order approximation.
The integrals in \eqref{eq:weakFormDefs} are computed using quadrature exact for 
polynomials of degree five to ensure the numerical scheme is third-order 
convergent.
We use the four-point Gauss-Lobatto quadrature rule since the function 
evaluations at the interval boundaries can be reused for the numerical fluxes 
$\bF$.

\subsection{Runge-Kutta time integration}
For a fully third-order method, we require an explicit time-stepping
scheme for \eqref{eq:ode1} that is at least third-order.
We use the 
standard SSP$(3,3)$ third-order strong stability-preserving (SSP) Runge-Kutta 
time discretization introduced in \cite{CWShu}.
%}
This specific Runge-Kutta method is a convex combination of forward Euler 
steps, a property which below helps us prove that the cell means of the 
internal stages are realizable.

A scheme of higher order could be achieved by increasing the degree $\order$ of 
the approximation space $V_h^k$ as well as the order of the Runge-Kutta 
integrator.
Unfortunately SSP-RK schemes with positive weights can at most be fourth order
\cite{Ruuth2004,Gottlieb2005}.
A popular solution is given by the so called 
Hybrid Multistep-Runge-Kutta SSP methods.
A famous method is the seventh-order hybrid method in \cite{Huang2009} while 
recently two-step and general multi-step SSP-methods of high order have been
investigated \cite{Ketcheson2011,Bresten2013}.




\subsection{Numerical optimization}
\label{sec:Optimization}

In order to evaluate $\bff(\U)$ and $\br(\U)$ on the spatial quadrature points 
in each Runge-Kutta stage, we first compute the multipliers
$\alphahat(\U)$ solving the dual problem \eqref{eq:dual}.
For the Maxwell-Boltzmann entropy the dual objective function and its gradient 
are
$$
f(\bsalpha) := \Vint{\exp(\basis^T \bsalpha)} - \U^T \bsalpha \quand
\bg(\bsalpha) = \Vint{\basis \exp(\basis^T \bsalpha)} - \U,
$$
respectively.

We use the numerical optimization techniques proposed in \cite{ahot2013}.
The stopping criterion for the optimizer is given by
$$
\| \bg(\bsalpha) \|_2 < \tau,
$$
where $\| \cdot \|_2$ is the Euclidean norm, and $\tau$ is a user-specified 
tolerance, and we also use the isotropic regularization technique to return 
multipliers for nearby moments when the optimizer fails.%
\footnote{The optimizer can fail for two reasons:  either the Cholesky 
factorization required to find the Newton direction fails or the number of 
iterations reaches a user-specified maximum $k_{\max}$.
}
Isotropically regularized moments are defined by the convex combination
$$
\bv(\bu, r) := (1 - r) \bu + r u_0 \uIso,
$$
where $\uIso = \frac12 \Vint{\basis}$ is the moment vector of the isotropic 
density $\phi(\mu) \equiv 1/2$.
The form of $\bv(\bu, r)$ is also chosen so that $\bv(\bu, r)$ has the same 
zeroth-order moment as $\bu$.
We define for an outer loop an increasing sequence $\{ r_m \}$ for $m = 0, 1, 
\ldots, m_{\max}$.  We begin at $m = 0$ with $r = r_0 := 0$ and only increment 
$m$ if the optimizer fails to converge for $\bv(\bu, r_m)$ after $k_r$
iterations.
It is assumed that $r_{m_{\max}}$ is chosen large enough that the optimizer 
will always converge for $\bv(\bu, r_{m_{\max}})$ for any realizable $\bu$. 

\subsection{Slope limiting}
A slope limiter $\Lambda$ is required to ensure the stability of the method and 
reduce non-physical oscillations in the solution.
We use the standard TVBM corrected minmod limiter proposed in 
\cite{CockburnShuV}.

Assuming that the major part of the spurious oscillations are 
generated in the linear part of the underlying polynomial, whose slope in
the $j$-th cell is 
simply $\Uhat_j^{(1)}$, a basic limiter can be defined as
\begin{align*}
 \Lambda^{\text{scalar}}_j(\Uhat) = \left\{ 
  \begin{array}{cc}
   \left( \begin{array}{c}
           \left( \Uhat^{(0)}_j \right)^T \\
           \left( D_j(\Uhat) \right)^T \\
           (0, 0, \ldots , 0)
          \end{array} \right)
    &\text{ if }
    \begin{array}{c}
     \abs{\Uhat_j^{(1)}} \geq M(\dx_j)^2 \text{ and,} \\
     D_j(\Uhat) \ne \Uhat_j^{(1)}
    \end{array} \\
    \Uhat_j & \text{otherwise}
  \end{array} \right.
\end{align*}
for the $j$-th cell,
where the absolute value and inequality are applied component-wise, and
\begin{align*}
 D_j(\Uhat) = D(\Uhat_{j - 1}, \Uhat_j, \Uhat_{j + 1}) := 
  m(\Uhat_j^{(1)}, \Uhat_{j + 1}^{(0)} - \Uhat_j^{(0)}, 
  \Uhat_j^{(0)} - \Uhat_{j - 1}^{(0)}).
\end{align*}
The label ``scalar'' is used because the limiter is directly applied to each 
scalar component of $\U_h$.
The function $m$ is the standard minmod function applied component-wise:
\begin{align*}
m(a_1,a_2,a_3) &= \begin{cases}
 \operatorname{sign}(a_1) \min\{|a_1|,|a_2|,|a_3|\} & \text{if } 
 \operatorname{sign}(a_1) = \operatorname{sign}(a_2) = 
 \operatorname{sign}(a_3), \\
0 & \text{else}.
\end{cases}
\end{align*}

The constant $M$ is a problem-dependent estimate of the second derivative, 
though we note that in \cite{CockburnShuIV} the authors did not find the 
solutions very sensitive to the value chosen for this parameter.

However, it has been found that applying the limiter to the components 
themselves may introduce non-physical oscillations around an otherwise monotonic 
solution \cite{Cockburn1989}.
Therefore we instead apply the limiter to the local characteristic fields of the 
solution.
The characteristic fields are found by transforming the moment vector $\U$ 
using the matrix $\bV_j$, whose columns hold the eigenvectors of the Jacobian 
$\partial \bff / \partial \U$ evaluated at the cell mean $\Ubar_j$.
We then transform back to the moment variables after applying the limiter.
In the end, since $\Uhat_j$ is a matrix of size $(\order + 1) \times (\nmom + 
1)$, this transformation is accomplished by post-multiplying with $\bV_j^{-T}$ 
so that
$$
 \Lambda_j(\Uhat) = \Lambda^{\text{scalar}}_j(\Uhat \bV_j^{-T}) 
\bV_j^T,
$$
where $\Uhat \bV^{-T}_j$ is understood as $(\ldots , \Uhat_{j - 1} \bV^{-T}_j, 
\Uhat_j \bV^{-T}_j, \Uhat_{j + 1} \bV^{-T}_j, \ldots)$.
We apply this limiter is applied to every Runge-Kutta stage.

The Jacobian is computed at the cell means $\Ubar_j$ using 
\eqref{eq:fluxJacobian}.
This indeed also implies that we must solve the dual problem \eqref{eq:dual} to 
compute $\alphahat(\Ubar_j)$ for each cell.

There are more advanced limiter strategies, for example WENO limiting 
\cite{Qiu2005,Zhao2013} or generalized minmod-limiting 
\cite{Krivodonova2004,Krivodonova2007}, removing the drawback of having a 
problem-dependent parameter $M$.
The slope limiter is however not a focus of this work.

\subsection{Realizability preservation and limiting}

In order to evaluate the flux-term $\bff(\U_j(t, x_{jq}))$ at the spatial quadrature nodes 
$x_{jq}$ in the $j$-th cell, we at least need $\U_j(t, x_{jq}) \in 
\RD{\basis}{}$ for each node, although when the angular integrals are 
approximated by quadrature, we in fact need $\U_j(t, x_{jq}) \in 
\RQ{\basis}$.
Unfortunately higher-order schemes typically cannot guarantee this, as
has been 
observed in the context of the compressible Euler equations (which are
indeed in the hierarchy of minimum-entropy models) in \cite{Zhang2012}.

We can, however, first show that, when the moments at the quadrature nodes are 
realizable, our DG scheme preserves realizability of the cell means 
$\Ubar_j(t)$ under a CFL-type condition.  
With realizable cell means available, we then apply a linear scaling limiter to 
each cell pushing $\U_j(t, x_{jq})$ towards the cell mean and thus into the 
realizable set for each node $x_{jq}$.

\subsubsection{Realizability preservation of the cell means}

To prove realizability preservation of the cell means we will need three main 
ingredients:  first, an exact quadrature to represent the cell means using 
point values from the cell; second, a representation of the moments collision 
operator; and finally a lemma that allows us to add the flux term without 
leaving the realizable set.

First, following \cite{Zhang2010,Zhang2011a}, we consider the 
$\nqs$-point Gauss-Lobatto rule and use its exactness for polynomials of degree 
$\order \le 2\nqs - 3$ to write the cell means as
\begin{equation}
 \Ubar_j(t) = \frac{1}{\dx} \int_{I_j} \U_j(t, 
  x) dx = \sum\limits_{q = 1}^{\nqs}w_q \U_{j}(t, x_{jq}),
\label{eq:cellMeanWithQuad}
\end{equation}
where $x_{jq} \in I_j$ are the quadrature nodes on the $j$-th cell, and $w_q$ 
are the weights for the quadrature on the reference cell $[-1/2, 1/2]$.
We choose the Gauss-Lobatto quadrature in particular because it includes the 
endpoints, that is
\begin{equation}
 x_{j - 1/2}^+ = x_{j1} \quand x_{j + 1/2}^- = x_{j\nqs}
\label{eq:GLquadEndPoints}
\end{equation}

Secondly, we note that since the collision kernel $T$ in
\eqref{eq:collisionOperator} is positive by assumption, the moments of the 
collision operator applied to the entropy ansatz can be written as the 
difference between a realizable moment vector $\UcollR(\U)$ and the given 
moment vector $\U$:
\begin{align}
\label{eq:CollisionOperatorMoments}
 \br(\U) = \Vint{\basis \collision{\ansatz_{\U}}} = \UcollR(\U) - \U.
\end{align}
For example, in the case of isotropic scattering ($T \equiv 1/2$), we have 
$\UcollR(\U) = u_0\uIso$.

Finally, we use the following lemma:
\begin{lemma} \label{lem:uPlusF}
If $\bu \in \RD{\basis}{}$ and $a - |b| \ge 0$, then $a\bu + b\bff(\bu) \in 
\RD{\basis}{}$.
\end{lemma}
\begin{proof}
Since $\bu \in \RD{\basis}{}$, then there exists a solution to the minimum 
entropy problem $\ansatz_{\bu}$, so that $\bu = \vint{\basis \ansatz_{\bu}}$ 
and $\bff(\bu) = \vint{\mu \basis \ansatz_{\bu}}$.  Thus
\begin{align*}
 a\bu + b\bff(\bu) &= \Vint{\basis \left( a + b\mu \right) \ansatz_{\bu}}.
\end{align*}
Since $\mu \in [-1, 1]$, the affine polynomial satisfies $a + b\mu \ge a - 
|b|$, so by assumption we have $(a + b\mu)\ansatz_{\bu} \ge 0$, which is a 
nonnegative measure representing $a\bu + b\bff(\bu)$.
\end{proof}

\begin{theorem}
\label{prop:eulerStepRealizable}
Assume $\source \ge 0$ and $2\nqs - 3 \ge k$, and let $\sig{t} := \sig{s} + 
\sig{a}$.
Consider the cell means at time instants $t^\timelvl$,
$$
\Ubar^\timelvl_j := \frac{1}{\dx} \int_{I_j} \U_j(t^\timelvl, x) dx.
$$
If the moment vectors $\U^\timelvl_{jq} := \U_j(t^\timelvl, x_{jq})$ at each spatial 
quadrature point $x_{jq}$ are in $\RD{\basis}{}$ (or $\RQ{\basis}$) and the 
CFL condition
\begin{align}
\label{eq:HO-CFL}
\frac{\dt}{\dx} < w_{\nqs}(1 - \sig{t}\dt).
\end{align}
holds, where $w_{\nqs}$ denotes the quadrature weight of the last quadrature 
weight of the $\nqs$-point Gauss-Lobatto quadrature rule on the reference cell 
$[-1/2, 1/2]$, then the cell means $\Ubar^{\timelvl + 1}_j$ computed by taking a 
forward-Euler time step for \eqref{eq:dweakform2} are also in $\RD{\basis}{}$ 
(respectively $\RQ{\basis}$).
\end{theorem}

\begin{proof}
The following arguments only use the fact that the realizable set 
is a convex cone, and therefore can be applied to either $\RD{\basis}{}$ or 
$\RQ{\basis}$ in exactly the same way.  For clarity of exposition, we also 
begin with the case $\source \equiv 0$.

By the orthogonality of our basis, $\Ubar_j(t) = \Uhat_j^{(0)}(t)$.  Therefore 
we use the subequations in \eqref{eq:weakform_m1} for $\Uhat_j^{(0)}$ (where, 
in particular we have $\partial_x \varphi_0 \equiv 0$).
We use the notation $\U_j^{\timelvl}(x) = \U_j(t^\timelvl, x)$, so that with a
forward-Euler approximation for the time derivative \eqref{eq:weakform_m1} gives
\begin{align*}
 \Ubar_j^{\timelvl + 1} = \Ubar_j^\timelvl + \dt &\left( 
 -\frac{\hat \bff(\U_j^\timelvl(x_{j + 1/2}^-),
  \U_{j + 1}^\timelvl(x_{j + 1/2}^+))
  - \hat \bff(\U_{j - 1}^\timelvl(x_{j - 1/2}^-), 
  \U_j^\timelvl(x_{j - 1/2}^+))}
  {\dx} \right. \\
  &\quad- \sig{a}\Ubar_j^\timelvl + \sig{s}\br(\U_j^\timelvl) \left.
  \vphantom{\frac12} 
\right).
\end{align*}
Now using the fact that the cell interfaces are the first and last 
quadrature nodes (recall \eqref{eq:GLquadEndPoints}), we now substitute the 
definition of $\hat \bff$ and the appropriate representation of the moments of 
the collision operator \eqref{eq:CollisionOperatorMoments}, then use the 
quadrature formula for the cell means \eqref{eq:cellMeanWithQuad}, and finally 
collect terms to get:
\begin{subequations}
\label{eq:uNplus1}
\begin{align}
 \Ubar_j^{\timelvl + 1} =& \Ubar_j^\timelvl + \dt \left( 
  -\frac{1}{2\dx} \left(
  \bff\left(\U^\timelvl_{j\nqs}\right) + \bff\left(\U^\timelvl_{(j + 1)1}\right)
  - \left(\U^\timelvl_{(j + 1)1} - \U^\timelvl_{j\nqs}\right) \right. \right.
  \nonumber \\
 &\qquad\qquad - \left. \left(\bff\left(\U^\timelvl_{(j - 1)\nqs}\right) + 
  \bff\left(\U^\timelvl_{j1}\right) - \left(\U^\timelvl_{j1}
  - \U^\timelvl_{(j - 1)\nqs}\right)\right) \right) \nonumber \\
 &\qquad\qquad - \sig{a}\Ubar_j^\timelvl + \sig{s}(\UcollR(\U_j^\timelvl)
  - \Ubar_j^\timelvl) \left. 
  \vphantom{\frac12} \right) \nonumber \\
 =& \sum\limits_{q = 1}^{\nqs}w_q \U^\timelvl_{jq} + \dt \left( 
  -\frac{1}{2\dx} \left(
  \bff\left(\U^\timelvl_{j\nqs}\right) + \bff\left(\U^\timelvl_{(j + 1)1}\right)
  - \left(\U^\timelvl_{(j + 1)1} - \U^\timelvl_{j\nqs}\right) \right. \right.
  \nonumber \\
 &\qquad\qquad\qquad\qquad - \left. \left(\bff\left(\U^\timelvl_{(j - 1)\nqs}
  \right) + 
  \bff\left(\U^\timelvl_{j1}\right) - \left(\U^\timelvl_{j1}
  - \U^\timelvl_{(j - 1)\nqs}\right)\right) \right) \nonumber \\
 &\qquad\qquad\qquad\qquad - \sig{t}\sum\limits_{q = 1}^{\nqs}w_q
  \U^\timelvl_{jq} + 
  \sig{s}\UcollR\left(\U_j^\timelvl\right) \left. \vphantom{\frac12} \right) 
  \nonumber \\
 =& \sum\limits_{q = 2}^{\nqs - 1} w_q (1 - \dt\sig{t}) \U^\timelvl_{jq} + \dt 
  \sig{s}\UcollR\left(\U_j^\timelvl\right) \label{eq:uNplus1-1} \\
 &+ \frac{\dt}{2\dx} \left( \U^\timelvl_{(j + 1)1}
  - \bff\left(\U^\timelvl_{(j + 1)1} \right) 
  + \U^\timelvl_{(j - 1)\nqs} + \bff\left(\U^\timelvl_{(j - 1)\nqs} \right)
  \right) \label{eq:uNplus1-2} \\
 &+ \left( w_1 - \frac{\dt}{2\dx} - \dt\sig{t}w_1 \right) \U^\timelvl_{j1} + 
  \frac{\dt}{2\dx}\bff\left( \U^\timelvl_{j1} \right) \label{eq:uNplus1-3} \\
 &+ \left( w_{\nqs} - \frac{\dt}{2\dx} - \dt\sig{t}w_{\nqs} \right) 
  \U^\timelvl_{j\nqs} - \frac{\dt}{2\dx}\bff\left( \U^\timelvl_{j\nqs} \right)
  \label{eq:uNplus1-4}
\end{align}
\end{subequations}
Keeping in mind that we have assumed that each moment vector $\U^\timelvl_{jq}$ 
is realizable, we consider each of the final lines:
\begin{itemize}
 \item If $\sig{t} \dt < 1$, a condition which is indeed weaker than 
  \eqref{eq:HO-CFL}, the expression in the first line, \eqref{eq:uNplus1-1}, is 
  a positive linear combination of realizable moments.  Since the realizable 
  set is a convex cone, this expression is realizable.
 \item The terms in the second line \eqref{eq:uNplus1-2} can be shown to be 
  realizable by two applications of \lemref{lem:uPlusF} with $a = 1$ and $b = 
  \pm 1$.
 \item The expressions in the last line, \eqref{eq:uNplus1-3} and 
  \eqref{eq:uNplus1-4}, are each realizable according to \lemref{lem:uPlusF} 
  and \eqref{eq:HO-CFL} (and recalling that $w_1 = w_{\nqs}$).
\end{itemize}
Finally, $\Ubar_j^{\timelvl + 1}$ is realizable since it is a sum of realizable 
moment vectors.

When $\source \ge 0$, notice that this simply adds to \eqref{eq:uNplus1}
the term $\vint{\basis \source}$, which is realizable and thus does not
affect the conclusion.
\end{proof}

Since we are using SSP-Runge-Kutta time-stepping schemes, whose stages are 
convex combinations of forward Euler steps, \thmref{prop:eulerStepRealizable} 
guarantees that under the appropriate CFL condition, the cell means for every 
Runge-Kutta stage are realizable.
In particular, the SSP(3, 3) which we use is a convex combination of Euler 
steps all with time step $\dt$.

%\begin{remark}
%If the scattering and absorption interaction coefficients are not piecewise 
%constant but rather in $V^k_h$ (or should be approximated in this space), then 
%to get a $\order$-th-order approximation of the term
%$$
%\frac{1}{\dx} \int_{I_j} \sig{a}(t, x) \U_j(t,  x) dx
%$$
%(and the corresponding term with $\sig{s}$), we need to use a Gauss-Lobatto 
%quadrature rule of order $2\nqs-3\geq 2\order$.  In this case, $w_{\nqs}$ would 
%be smaller and therefore lead to a more restrictive CFL condition.
%\end{remark}
%}{
%% nothing in short version
%}


\longpaper{
\begin{remark}
As in \cite{AllHau12} we need to modify the CFL condition a little bit more. 
Since we don't solve the optimization/closure problem analytically we make some 
numerical error, compare Section \ref{sec:NumQuad}.

For now, let $\psi_{j,\beta}$ be the (unknown) analytical solution of the 
optimization problem at quadrature point $x_\beta$ and $\hat\psi_{j,\beta}$ the 
approximative solution. Their moments are denoted accordingly by $\U_{j,\beta}$ 
and $\hat\U_{j,\beta}$, respectively. In the above proof we need to replace  
$\psi_{j,\beta}$ by the corresponding approximate solution $\hat\psi_{j,\beta} 
= \gamma_{j,\beta}\psi_{j,\beta}$ with $\gamma_{j,\beta} = 
\cfrac{\hat\psi_{j,\beta}}{\psi_{j,\beta}}$ an error indicator for the closure 
problem at quadrature point $\hat{x}_{j,\beta}$. Now, the last line of the 
proof has the form
\begin{align*}
\Xi_j^{(\timelvl)} 
&\hspace{-2pt}\geq\hspace{-5pt}\sum\limits_{\beta=2}^{\nqs-1}\hat{w}
_\beta\left(1-\dt\gamma_{j,\beta}\left(\sigma_{a,j,\beta}+\collconst_{j,\beta}
\right)\right) \psi_{j,\beta}^{(\timelvl)} + 
\left(\hat{w}_1\left(1-\dt\gamma_{1,\beta}\left(\sigma_{a,1,\beta}+\collconst_{1
,\beta}\right)\right)\right) \psi_{j-\frac12}^+
\\&\hskip 0.5cm -\gamma_{1,\beta}\frac{\dt}{\dx} \psi_{j-\frac12}^++ 
\left(\hat{w}_\nqs\left(1-\gamma_{\nqs,\beta}\dt\left(\sigma_{a,\nqs,\beta}
+\collconst_{\nqs,\beta}\right)\right)-\gamma_{\nqs,\beta}\frac{\dt}{\dx}
\right) \psi_{j+\frac12}^-
\end{align*}
Now the corresponding CFL condition reads
\begin{align}
\label{eq:HOCFL2}
\gamma\Delta t < \cfrac{\hat{w}_1\Delta 
x}{\left(\sigma_{a,\max}+\collconst_{\max}\right)\hat{w}_1\Delta x + 1}
\end{align}
where $\gamma = \max\limits_{j=1,\ldots \ncells}\{\gamma_{j\pm\frac12}^\mp\}$.
\end{remark}
}{
% nothing in short version
}

\subsubsection{Realizability-preserving Limiter}
\thmref{prop:eulerStepRealizable} makes the assumption that the 
point-values of the local DG polynomials are realizable. This can be achieved 
by applying a linear scaling limiter in each cell.
Recall the definition of $\U_j(t, x)$:
\begin{align*}
 \U_j(t, x) = \sum\limits_{i=0}^{\order}\Uhat_j^{(i)}(t) \varphi_i 
  \left(\frac{x - x_j}{\dx}\right) = \bar{\U}_j(t) + \sum\limits_{i=1}^{\order} 
  \Uhat_j^{(i)}(t) \varphi_i \left( \frac{x - x_j}{\dx} \right).
\end{align*}
We can see that using convexity of the realizable set, if $\Ubar_j$ is 
realizable, then for each quadrature point there exists a $\theta \in 
[0,1]$ such that
\begin{align*}
 \U_j^\theta(t, x_{jq}) := \theta \Ubar_j(t) + (1 - \theta) \U_j(t, x_{jq})
\end{align*}
is realizable.  Indeed, by inserting the definition of $\U_j(t, x_{jq})$ from 
above, we can write the limited moment vector as
\begin{align*}
 \U_j^\theta(t, x_{jq})
  = \Ubar_j(t) + (1 - \theta) \sum\limits_{i = 1}^{\order} 
  \Uhat_{j}^{(i)}(t) \varphi_i\left( \frac{x_{jq} - x_j}{\dx} \right);
\end{align*}
thus when limiting is necessary, the higher-order coefficients
are damped while the cell mean remains unchanged.
An example of the limiting process is illustrated in 
\figref{fig:QuadLimiterEx1}, which considers the following polynomial 
representation of an M${}_1$ solution:
$$
\begin{pmatrix} u_0\\u_1 \end{pmatrix} 
 = \begin{pmatrix} 1 & 0.5 &-0.2\\0.8 & 0.2 & 0.6 \end{pmatrix}
 \begin{pmatrix} 1 \\ 2x \\  \frac12(12x^2-1) \end{pmatrix}
$$

After limiting with $\theta > 9/11$ the vector $(u_0^\theta, 
u_1^\theta)$ becomes realizable.

\begin{figure}
\centering
\subfloat[Before limiting; notice the nonrealizable moments at the end points]
{\externaltikz{LimiterM1_1}{\resizebox{0.47\textwidth}{!}
{\input{Images/M1Limit1.tex}}}}
\subfloat[After limiting; realizable]
{\externaltikz{LimiterM1_2}{\resizebox{0.47\textwidth}{!}
{\input{Images/M1Limit2.tex}}}}
\caption{Application of the realizability preserving limiter to the M${}_1$ 
system for a quadratic polynomial.  Here, $(u_0, u_1)$ are realizable only if 
$|u_1| < u_0$. Black squares indicate the spatial quadrature points $x_q$.}
\label{fig:QuadLimiterEx1}
\end{figure}


Since the full realizable set $\RD{\basis}{}$ is characterized by the 
positive-definiteness of the associated Hankel matrices, computing the smallest 
$\theta$ such that $\U_j^\theta(t, x_{jq}) \in \RD{\basis}{}$ is in general 
difficult.
Furthermore, the realizable set for higher-dimensional problems (when 
dimension of the angular domain is more than one) is in general not 
well-understood.

This computation is however much easier for the numerical realizable set 
$\RQ{\basis}$ using its half-space representation.
This representation is also intriguing because it extends to 
higher-dimensional problems, since even in these cases $\RQ{\basis}$ remains 
the interior of a cone generated by a convex polytope.

In the following
for clarity of exposition we omit the time arguments and 
spatial-cell indices, therefore using $\Ubar$ to indicate the (always 
realizable) moment vector at the cell mean and $\U_q$ to indicate the (not 
necessarily realizable) moment vector at a quadrature point.
In an implementation, the limiter is applied to every quadrature point
in every cell.

%\paragraph{Facet-based representation}
If we assume that the moment vectors $\Ubar$ and $\U_q$ 
have been scaled such that $\max(\bar{u}_0, 
u_{q0}) = 1/2$, where $u_{q0}$ is the zero-th component of $\U_q$,%
\footnote{
Here we are using $1/2$ instead of $1$ to ensure that $\Ubar$ and $\U_q$ are 
in the \textit{interior} of $\RQsone{\basis}$.
}
then the limited moment vector $\U_q^\theta := \theta \Ubar + (1 - \theta) 
\U_q$ satisfies $u^\theta_{q0} < 1$
for all $\theta \in [0, 1]$.
Therefore we can work without loss of generality with $\RQsone{\basis}$, which 
(like $\RQone{\basis}$ but unlike the unbounded $\RQ{\basis}$)
is the interior of a convex  polytope:
$$
\RQsone{\basis} =  \operatorname{int}\operatorname{conv}(\RQone{\basis}\cup 
\{0\})
$$

Next we use that convex polytopes have the following \textit{half-space 
representation} \cite{brondsted-convex-polytopes}
$$
 \RQsone{\basis} = \left\{ \U \in \R^{\nmom + 1}:~ \ba_i^T\U < b_i, i \in \{1, 
\ldots, d\} \right\},
$$
where $d$ is the number of facets of the polytope.
To compute where the line from $\Ubar$ to $\U_q$ intersects the boundary 
of the realizable set $\partial \RQsone{\basis}$, we first compute for each 
facet
$$
 \ba_i^T(\theta_{qi} \Ubar + (1 - \theta_{qi}) \U_q) = b_i
 \quad \iff \quad
 \theta_{qi} = \frac{b_i - \ba_i^T\U_q}{\ba_i^T(\Ubar - \U_q)}.
$$
If we wanted to limit exactly to $\partial \RQ{\basis}$, we would first take
$$
\theta_q^{\partial \cR} := \begin{cases}
             0 & \text{if there is no } \theta_{qi} \in [0, 1], \\
             \max\{\theta_{qi} : \theta_{qi} \in [0, 1] \} & \text{else;}
            \end{cases}
$$
and then for the cell in question, we would apply the largest $\theta_q$ from 
the quadrature nodes:
$\theta^{\partial \cR} := \max\{\theta_q^{\partial \cR}\}$.
This would ensure that the moment vectors at each quadrature node in the cell 
are in the realizable set or on its boundary.

In practice, however, we do not want to choose $\theta_q$ such that the limited 
moment vector $\theta_q \Ubar + (1 - \theta_q) \U_q$ lies exactly on the 
boundary of the realizable set $\partial \RQ{\basis}$, but rather so that 
the limited moment vector is in the interior of $\RQ{\basis}$.
Therefore we define a tolerance $\eps$ to add to each relevant $\theta_{qi}$ 
(that is in $[0, 1]$) as well as those facets such that $\theta_{qi} \in [-\eps, 
0]$, indicating that while $\U_q$ is on the correct side of the half space, it 
is closer than $\eps$ to the facet.
Keeping in mind that $\theta_q$ should not exceed one, this gives
$$
\theta_q := \begin{cases}
             0 & \text{if there is no } \theta_{qi} \in [-\eps, 1], \\
             \min \{ 1, \eps + \max\{\theta_{qi} : \theta_{qi} \in [-\eps, 1] \} 
              \} & \text{else.}
            \end{cases}
$$
Finally, in the implemented version, for the cell we set $\theta = \max \{ 
\theta_q \}$.
Figure \ref{fig:QuadLimiter} shows an example for the full moment model with 
$\nmom=2$.

\InsertFig{
\subfloat[Limiter example for $\nmom=2$ full moments $\mbasis$-basis with
$\nqmu = 7$ and, for simplicity of exposition, $u_{q0} = 
\bar{u}_0 = 1$.\label{fig:QuadLimiter}]
{\resizebox{0.45\textwidth}{!}
{\externaltikz{QuadratureLimiter}{\input{Images/QuadratureLimitertikz.tex}}}}%
%
\hspace{0.05\textwidth}%
%
\subfloat[The number of facets of $\RQ{\basis}$ for a few $\MN$ (for
$N \in \{4, 6, 8\}$) and $\MMN$ (for $N \in \{2, 3, 4\}$) models.
The number of facets of MM$_2$ and MM$_3$ are almost exactly the
same.
\label{fig:Facets}]
{
\includegraphics[scale=0.4]{Images/facets-MvsMM}
}

}{}{}

The main drawback to this implementation of the limiter is that, as
illustrated 
in \figref{fig:Facets} the number of facets $d$ grows rapidly both with 
the number of moments $\nmom$ and the number of quadrature points $\nqs$.
The numbers for this figure were computed using results from the study
of convex polytopes, and
a more detailed discussion is in the appendix.
This issue was not a significant obstacle for our simulations but will be for 
simulations in higher dimensions where a much larger number of quadrature 
points will be necessary.
One clear speed up is that not every $\theta_{qi}$ should be computed, as many 
facets do not intersect the line between $\Ubar$ and $\U_q$.
More importantly, however, an implementation in higher-dimensions will probably 
have to further approximate $\RQ{\basis}$ by removing some irrelevant facets.

%We leave this to future work, but quickly note here that the monomial case  
%is actually the worst-case scenario:  a celebrated theorem in the study of 
%convex polytopes states that the number of facets of $\RQone{\mbasis}$, 
%commonly known as the cyclic polytope, provides an upper bound for the possible 
%number of facets of any convex polytope with a given number of vertices 
%\comment{for graham: make more precise and give a ref!!}.

\longpaper{
\paragraph{Vertex-based representation}
\comment{Complexity is $\mathcal{O}(n^{3.5})$ if $n$ is the dimension of the
solution vector, using Karmarkas algorithm \cite{hamacher2006linear}}
\comment{OK sounds good, but I'll check with my old advisor anyway.}
For $\nmom$ reasonably big it may be more appropriate to solve the limiter 
problem in the vertex-based representation of the polytope using the original 
definition of realizability \eqref{eq:QRealizable}:
\begin{subequations}
\label{eq:LP}
	\begin{align}
\min\quad&\theta&&&	\min \quad&c^T\nu\\
	s.t.\quad &\sum\limits_{i=1}^{\nqmu}\lambda_i\basis(\mu_i) 
=(1-\theta)\bu+\theta\bar{\bu}&\Longleftrightarrow&&s.t. \quad &A\nu = \bu\\
	&\theta,\lambda_i\geq 0&&&&\nu\geq 0
	\end{align}
	\end{subequations}
	with $\nu = \begin{pmatrix}
	\lambda\\\theta
	\end{pmatrix}$, $c = (0,\ldots,0,1)^T$ and $A = \begin{pmatrix}
	M&\bu-\bar{\bu}
	\end{pmatrix}$ with $M_{ij} = \basis_i(\mu_j)$.
Dualizing this linear program (to avoid the equality constraints) gives 
\cite{hamacher2006linear}

\begin{subequations}
\label{eq:DLP}
\begin{align}
	\max\quad&\omega^T\bu\\
	s.t.\quad &\omega^TA\leq c
	\end{align}
	\end{subequations}
	

Using the strong duality theorem \cite{hamacher2006linear} we get that for an 
optimal solution of \eqref{eq:DLP} and \eqref{eq:LP} satisfy $\theta = c^T\nu = 
\omega^T\bu$

Therefore solving the dual LP gives immediately the optimal value for $\theta$. 
Note that it is again helpful to choose normalized moments for numerical 
stabilization of the problem. 
\longpaper{
This results in the following algorithm:

\begin{algorithm}[H]
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \Input{$\U = \left(u_0,\ldots,u_{\Nmom-1}\right)\in\R^{\Nmom}$, $\bar{\U} = 
\left(\bar{u}_0,\ldots,\bar{u}_{\Nmom}\right)\in\R^{\Nmom}$ realizable, safety 
factor $\eps$}
  \Output{$\hat{\U}$ realizable}
  \BlankLine
  Set $\phi = \cfrac{\U}{\max(u_0,\bar u_0)}$, $\bar{\phi} = 
\cfrac{\bar{\U}}{\max(u_0,\bar u_0)}$\;
  Set $c = (0,\ldots,0,1)^T$ and $A = \begin{pmatrix}
  	M&\phi-\bar{\phi}
  	\end{pmatrix}$ with $M_{ij} = \basis_i(\mu_j)$\;
  Solve \eqref{eq:DLP} for $y$\;
 \If{$\theta>0$}{
   $\theta = \min(\theta+\eps,1)$\;}
  Set $\hat{\U} = \left(\theta \bar{\U} + (1-\theta)\U\right)$\;
  \caption{DLP-Limiter for quadrature based algorithms.}\label{alg:DLPLimiter}
\end{algorithm} %\DecMargin{1em}
}{}


Here we only have a polynomial number of variables in this linear program but 
we can't precompute the solution efficiently. However, for large $\nmom$ this 
is still more efficient than the facet-based limiter.
\comment{That is true. But it is clear that there is an $N$ where this
intersects. I bet that this is indeed relevant in higher dimension.}
\comment{Sure, but if we're going to include this section, I still think we 
should include some kind of experiments or discussion about whether this 
intersection point is reasonably close.  And anyway, I don't think this will be 
hard to do.}
\comment{I agree.}
}{}
